Satellite Image and Machine Learning based Knowledge Extraction in the Poverty and Welfare Domain

Recent advances in artificial intelligence and machine learning have created a step change in how to measure human development indicators, in particular asset based poverty. The combination of satellite imagery and machine learning has the capability to estimate poverty at a level similar to what is achieved with workhorse methods such as face-to-face interviews and household surveys. An increasingly important issue beyond static estimations is whether this technology can contribute to scientific discovery and consequently new knowledge in the poverty and welfare domain. A foundation for achieving scientific insights is domain knowledge, which in turn translates into explainability and scientific consistency. We review the literature focusing on three core elements relevant in this context: transparency, interpretability, and explainability and investigate how they relates to the poverty, machine learning and satellite imagery nexus. Our review of the field shows that the status of the three core elements of explainable machine learning (transparency, interpretability and domain knowledge) is varied and does not completely fulfill the requirements set up for scientific insights and discoveries. We argue that explainability is essential to support wider dissemination and acceptance of this research, and explainability means more than just interpretability.

==> Satellite Imaging and XAI (3)/table-4.tex <==
\begin{landscape}
\footnotesize
\begin{center}
\begin{longtable}{|p{1cm}|p{1cm}|p{8cm}|p{11.5cm}|}
  \caption{A list of all reviewed papers including comments on methods and data used.} \label{table:summary}\\
  \hline 
  Ref. & Year & Method & Data \\ 
  \hline
\citep{AngeliniEtAl2019} &
2019 &
Support Vector Machines (SVM) and k-Nearest-Neighbors (kNN).
&
Input: Several computed features from low resolution Sentinel-2 satellite images.
Output: Publically available Afrobarometer survey responses for Kenya, Nigeria, and Tunisia. Infrastructure, living conditions, perception of government corruption.
\\ \hline
\citep{AyushEtAl2020}
&
2020
&
Gradient descent boosting trees, but using deep neural networks (Yolov3) for object detection in the feature generation step.
&
Input: xView (DigitalGlobe) high resolution satellite images. Features are extracted from these using Yolov3.
Target: Living Standards Measurement Study for Uganda. Consumption expenditure.
\\ \hline
\citep{AyushEtAl2021}
&
2021
&
Gradient descent boosting trees. Deep neural networks (Yolov3) for object detection in the feature generation step. Reinforcement learning method for selecting low-resolution or high-resolution images.
&
Input: xView (DigitalGlobe) high resolution satellite images and low resolution Sentinel-2 satellite images.
Target: Living Standards Measurement Study for Uganda. Consumption expenditure.
\\ \hline
\citep{BabenkoEtAl2017}
&
2017
&
GoogleNet Convolutional Neural Network(CNN) model. Trained directly to predict poverty.
&
Input: Digital Globe and Planet satellite imagery (RGB). High res and low res.
Target: Survey data from the 2014 MCS-ENIGH. Income per adult equivalent. Three poverty groups (fraction of households living in poverty). Poverty lines.
\\ \hline
\citep{Chen2016}
&
2016
&
First, ResNet50 Convolutional Neural Network (CNN) model trained on ImageNet.
The second step is done with linear ridge regression.
&
Input: First, 8 bands from year-averaged landsat-7 satellite images. Second, the features from the CNN.
Target: First, night time lights. Second, a normalized wealth score computed from survey data collected by the World Bank in the Living Standard Measurement Study (LSMS).
\\ \hline
\citep{EngstromHN2021}
&
2021
&
Features are identified using a combination of Convolutional Neural Network (CNN) and classification of spectral and textural characteristics. In some cases (roads) is manual identification used. 
Finally a linear LASSO model that uses the features as input.
&
Input: Object and texture features derived from HSRI (High Spatial Resolution Imagery). 
Target: Household estimates of per capita consumption imputed into the 2011 Census of population and housing  (Sri Lanka).
\\ \hline
\citep{EngstromEtAl2019}
&
2019
&
Linear regression (LASSO) for selecting the 15 most important features. Random Forest regression for the poverty index.
&
Input: Quickbird-2 multispectral (Blue, Green, Red, and Near-Infrared) satellite images. Several features are computed from these.
Target: The Ghana Living Standards Survey Round Six (2012-2013). The 2010 Population and Housing Census gathered information from each household on September 26, 2010 (Accra). Neighborhood poverty rates, slum index.
\\ \hline
\citep{HeadEtAl2017}
&
2017
&
VGG16 Convolutional Neural Network (CNN), pre-trained on ImageNet but fine-tuned with night time lights.
&
Input: Satellite images from Google Static Maps. “Low res”. NOAA nighttime light images from the DMSP-OLS website are used for fine-tuning.
Target: Demographic and Health Surveys (DHS) data. Several indices from these.
\\ \hline
\citep{IrvinLR2017}
&
2017
&
Tries both “standard” Convolutional Neural Network (CNN) and a ResNet CNN network. Tries both training the ResNet from scratch and having one pre-trained on ImageNet data but fine-tuned on their task. Tests with averaging outputs from image tiles, or using more advanced recurrent neural networks for combining (LSTM).
&
Input: Satellite images from Google Maps Static API, zoom level 15.
Target: Demographic and Health Surveys (DHS) data. Poverty prediction with wealth index, split into 4 categories. Malnutrition prediction using height and weight for age scores, split into 6 categories.
\\ \hline
\citep{IrvineWM2017}
&
2017
&
A k-Nearest-Neighbor (kNN) model with k=3. Several features computed from the satellite images.
&
Input: Satellite image data from the National Geospatial-Intelligence Agency (NGA). Commercial data and sometimes four spectral bands. Features (color indices, objects, …) computed from this.
Target: Survey responses collected in sub-Saharan Africa by the Afrobarometer network in its Round 4 (2008/2009) surveys.
\\ \hline
\citep{JeanEtAl2016}
&
2016
&
The VGG-F Convolutional Neural Network (CNN) pre-trained on ImageNet data, fine tuned on night time lights. Ridge regression used for the final model from CNN features to poverty/well-being indices.
&
Input: Satellite image data from Google Static Maps API, zoom level 16 (several zoom levels are tried).
Target: Two are used. Consumption expenditure as measured in the World Bank’s Living Standards Measurement Surveys (LSMS). Expenditures are averaged over clusters and the log expenditure is modeled. Household asset score taken from the Demographic and Health Surveys (DHS).
\\ \hline
\citep{KimEtAl2016}
&
2016
&
ResNet-50 Convolutional Neural Network (CNN) pre-trained on ImageNet and then tuned on night time lights.
&
Input: Satellite image data from Google Static Maps API, zoom level 14, 16 and 18 (all three levels are used).
Target: Asset wealth index computed from the Demographic and Health Surveys (DHS).
\\ \hline
\citep{LeeB2020}
&
2020
&
XGBoost (decision tree) for the feature based model. Convolutional Neural Network (CNN) for the satellite image based model.
&
Input: OpenStreetMap data, the Visible Infrared Imaging Radiometer Suite Day/Night Band (VIIRS DNB) nighttime lights dataset, day-time satellite images (Google Static Map, zoom level 16), and the High-Resolution Settlement Layer (HRSL) datasets
Target: The International Wealth Index (IWI) computed from the Demographic and Health Surveys (DHS) data.
\\ \hline
\citep{LiEtAl2019}
&
2019
&
Gaussian process with Radial Basis Function (RBF) kernel, Stochastic gradient boosting, Partial Least Squares (PLS) regression for generalized linear models, Random Forest (RF), Rotation forest, Support Vector Machine (SVM), Neural network with feature extraction
&
Input: Imagery from version 4 of the 2010 night-time lights by the DMSP/OLS satellites. Several features calculated from these images.
Target: High or low poverty county, as defined by the Chinese government.
\\ \hline
\citep{NiEtAl2020}
&
2021
&
Convolutional Neural Networks (CNNs). Four pre-defined architectures: VGG-Net, Inception-Net, ResNet and DenseNet. The two latter were also modified and tested as two new models.
&
Input: Satellite images from Google Maps Static API. Fine tuning with night-time light imagery from DMSP/OLS satellite.
Target: Demographic and Health Survey (DHS) data. Poverty index. Unclear what type.
\\ \hline  
\citep{NjugunaM2017}
&
2017
&
Linear model of the log(MPI).
&
Input: Four features computed by combining three data sources. Mobile phone call detail records (CDRs). Night-time lights from the National Oceanic and Atmospheric Administration (NOAA). Population density estimates from the Landscan population database produced by US Department of Energy, Oak Ridge National Library.
Target: The multi-dimensional poverty index (MPI) calculated by the National Institute of Statistics in Rwanda (NISR) using data from the 2012 Rwanda Population and Housing Census (RPHC4).
\\ \hline
\citep{PandeyAK2018}
&
2018
&
Convolutional neural network (CNN) architecture for the first task. Trained from scratch. For the second task a multilayer perceptron.
&
Input: First, satellite images from Google Static Maps API, zoom level 16. Images only of villages. Second,  predicted roof material, source of lighting, and source of drinking water.
Target: First, the roof material, source of lighting, and source of drinking water in a region. In a second model, the household income level in a region. The information comes from the 2011 Census of India and Socio-Economic Caste Census of 2011.
\\ \hline
\citep{PerezEtAl2017}
&
2017
&
Convolutional Neural Network (CNN) of type ResNet and VGG-Net. Pre-trained on ImageNet data for RBG-bands, otherwise trained from scratch.
Try both gradient boosted trees and linear ridge regression for predicting AWI from the CNN features, and also (as comparison) directly from night-time light values.
&
Input: First, multispectral satellite imagery from Landsat 7 (several spectral bands tried). Second, CNN features.
Target: First, predicting class of night-time lights (3 classes). Second, Asset Wealth Index (AWI) from Demographic and Health Surveys (DHS) data.
\\ \hline
\citep{PerezEtAl2019}
&
2019
&
Convolutional Neural Network (CNN) with weighted Generative Adversarial Network (WGAN), for the first step. The second step is done with ridge regression.
&
Input: First, multispectral (9 bands) imagery from Landsat 7 (Enhanced Thematic Mapper Plus (ETM+)). RBG images are pan-sharpened (to get 15 m resolution). Second, the features from the CNN.
Target: It is not described fully what they train the CNN to predict, but it includes night-time lights. For a second, linear model, they use Asset Wealth Index (AWI) from Demographic and Health Surveys (DHS) data.
\\ \hline
\citep{PokhriyalJ2017}
&
2017
&
A model with one linear term and one nonlinear Gaussian Process term.
&
Input: Several features extracted from many different data sources; e.g., Open Street Map,  Mobile phone call records (CDRs), World Climate Database, the Digital Elevation Database, Night Time Lights, and the Soil and Terrain Database for Senegal.
Target: The Global Multidimensional Poverty Index (MPI), computed from Demographic and Health Surveys and Multiple Indicator Cluster Survey (DHS-MICS) data.
\\ \hline
\citep{SmithW2018}
&
2018
&
Linear model. The “unlit rural percentage” is used as an indicator for poor rural regions (100 square km regions).
&
Input: Night time lights from Defence Meteorological Satellite Program’s Operational Linescan System (DMSP-OLS). Population estimations from the Oak Ridge National Laboratory LandScan. By combining these is the “unlit rural percentage” (URP) computed.
Target: Comparative Wealth Index (CWI) and Unmet Basic Needs (UBN) from the Demographic and Health Surveys (DHS) data.
\\ \hline
\citep{SteeleEtAl2016}
&
2021
&
Hierarchical Bayesian Geostatistical Models (BGMs). Inputs are features computed from several data sources.
&
Input: Mobile phone call detail records (CDRs) from Telenor, partly for the same households as the market surveys in the input. VIIRS night-time lights. Population counts from CIESIN - Global Rural Urban Mapping Project. Climate indicators from CGIAR-CSI.Vegetation indices from MODIS MOD13A1. Features from Open Street Map. Land cover features from ESA GlobCover Project, IGBP MODIS MCD12Q1, and ONRL DAAC Synergetic Land Cover Product (SYNMAP).
Target: Three development indicators. The Wealth Index from Demographic and Health Surveys (DHS). The Progress out of Poverty Index based on a survey of adults in Bangladesh by InterMedia Financial Inclusion Insight Project in 2014. Two sequential large-scale market research household surveys run by Telenor.
\\ \hline
\citep{SubashKA2018}
&
2018
&
Artificial Neural Network (unspecified architecture). 
&
Input: Night time lights from India Lights API, and GDP values from India statistics.
Target: Poverty estimates from India survey.
\\ \hline
\citep{TanEtAl2020}
&
2020
&
ResNet50 (CNN) for the first task. Ridge regression for the second task.
&
Input: First, Landsat 8 images. Second, the features from the ResNet50 network. 
Target: First, spectral index data (NDVI, MNDWI, and NDBI), and night-time light data (Suomi NPP). Second, development indicators from the Chinese statistical yearbook data.
\\ \hline
\citep{TingzonEtAl2020}
&
2020
&
Pixel-wise modeling. Three models tried: logistic regression, linear support vector machines (SVM), and random forest (RF).
&
Input: Sentinel 2 satellite data, from these were 66 features computed per pixel.
Target: Field data of informal migrant settlements collected by the humanitarian organization iMMAP in 2019.
\\ \hline
\citep{WatmoughEtAl2019}
&
2019
&
Classification decision tree. Image features are computed from the satellite images using a combination of object-based image classification, fuzzy classification, and Random Forest (RF).
&
Input: Features computed from two satellite sources: land use/land cover (LULC) map derived from a QuickBird image, and Moderate Resolution Imaging
Spectro-radiometer (MODIS) data.
Target: A wealth index designed by the authors based on household survey data collected by the authors.
\\ \hline
\citep{WatmoughEtAl2016}
&
2016
&
Random Forest (RF).
&
Input: Satellite data from Landsat Enhanced Thematic Mapper Plus (ETM+) and the MODIS Normalized Difference Vegetation Index (NDVI). Features were computed from these.
Target: A welfare index computed from socioeconomic data at the community level from the 2001 Indian National Population and Household Census.
\\ \hline
\citep{WuT2019}
&
2019
&
First, ResNet50 model pre-trained on ImageNet data, fine tuned on night-time light data. Second, linear ridge regression.
&
Input: First, LANDSAT 8 images. Second, the features from the ResNet50 model.
Target: First, Nighttime light data (Suomi NPP satellite). Second, Gross domestic product (GDP) and total retail sales of consumer goods (TRSCG).
\\ \hline
\citep{XieEtAl2016}
&
2016
&
First, the VGG-F Convolutional Neural Network (CNN) model, pre-trained on ImageNet. Second, logistic regression.
&
Input: First, satellite images from the Google Static Maps API, at zoom level 16. Second, the features from the CNN.
Target: First, night time light intensities from The National Oceanic and Atmospheric Administration (NOAA). Second, data with binary poverty labels from Living Standards Measurement Study (LSMS) survey conducted in Uganda (Uganda Bureau of Statistics 2012).
\\ \hline
\citep{YehEtAl2020a}
&
2020
&
The ResNet-18 Convolutional Neural Network (CNN) model (v2, with preactivation). Pre-trained on ImageNet data. One network for daytime satellite images, one for night-time.
&
Input: Multispectral images from Landsat archives available on Google Earth Engine, and night-time lights images (VIIRS and DMSP).
Target: Wealth index from Demographic and Health Surveys (DHS) data.
\\ \hline
\citep{ZhaoEtAl2019}
&
2019
&
Random Forest (RF). A Convolutional Neural Network (CNN) VGG-F, trained on ImageNet data, was fine-tuned to predict night time light classes (and thus learn features).
&
Input: Night-time lights from the VIIRS Cloud Mask–Outlier Removed (vcm–orm) annual composite NPP-VIIRS DNB data (NOAA/NCEI). Google Static Maps satellite images, zoom level 16 (high resolution). Open Street Map. Land cover maps from the European Space Agency (ESA) Climate Change Initiative. Different features were computed from these.
Target: The Wealth Index (WI) from the Demographic and Health Surveys (DHS).
\\ \hline
%\label{table:summary}
\end{longtable}
\end{center}
\end{landscape}

